Channel Tracking for Wireless Energy Transfer: A Deep Recurrent Neural Network Approach

In this paper, we study channel tracking for the wireless energy transfer (WET) system, which is practically a very important, but challenging problem. Regarding the time-varying channels as a sequence to be predicted, we exploit the recurrent neural network (RNN) technique for channel tracking. Particularly, combining the deep long short-term memory (LSTM) RNN with the deep feedforward neural network, we develop a novel channel tracking scheme for the WET system, which estimates the channel state information (CSI) at the energy transmitter based on the previous CSI estimates, and the current and previous harvested energy feedback information from the energy receiver. Numerical results demonstrate the superior performance and effectiveness of the proposed scheme.

==> Tex/motivation.tex <==
The key idea of our proposed scheme is to regard the time-varying channels as a sequence and to predict the channels sequentially.
To this end, in this paper, we use the RNN technique.
Unlike the traditional feedforward neural networks (FNNs), the RNNs are particularly useful and effective to process a sequence of data due to the exploitation of internal state (or memory) that
captures the long-term dependency or temporal property of the sequential data.
To process the sequential data, in the naive (or vanilla) RNN,
the hidden state $\mathbf{s} (n)$ and the output $\mathbf{o} (n)$ at time step $n$ are calculated as
$\mathbf{s} (n) = \sigma_{s} \big(  \mathbf{W}_{s} \mathbf{i} (n) + \mathbf{U}_{s} \mathbf{s} (n-1) + \mathbf{b}_{s}  \big)$ and $\mathbf{o} (n) = \sigma_{o} \big(  \mathbf{W}_{o} \mathbf{s} (n) + \mathbf{b}_{o}  \big)$, respectively,
where $\mathbf{i} (n)$ is the input at time step $n$ and $\sigma_{j}$, $j \in \{ s, o \}$, are the activation functions.
Also, $\mathbf{W}_{j}$, $j \in \{ s, o  \}$, and $\mathbf{U}_{s}$ are the weight matrices
and $\mathbf{b}_{j} $, $j \in \{ s, o  \}$, are the bias vectors. Note that the same activation functions and the same set of parameters are used at every time step.


The RNNs can be trained by the algorithm called the back-propagation through time (BPTT),
which can be considered as a generalization of the back-propagation algorithm used to train the FNNs.
However, the naive (deep) RNN trained with the BPTT turns out to be neither effective nor successful in learning the long-term dependency or temporal property of the sequential data
due to the vanishing/exploding gradient problem.
Also, it requires very high computational complexity to compute the gradients.
To address this critical issues, in this paper, we utilize an advanced RNN, called the LSTM, for the channel tracking.
%LSTM RNN has been widely and successfully applied in language modeling [22], machine translation [23], image captioning [24], and handwriting generation [25].
Unlike to the naive RNN, the LTSM is able to efficiently and effectively learn the long-term dependency of the sequential data
with the following three additionally introduced gates: the forget gate $\mathbf{g}_{f} (n)$, the input gate $\mathbf{g}_{i} (n)$, and the output gates $\mathbf{g}_{o} (n)$,
which are given by
\begin{align}
\mathbf{g}_{j} (n) = \sigma_{j} \big(  \mathbf{W}_{j} \mathbf{i} (n) + \mathbf{U}_{j} \mathbf{s} (n-1) + \mathbf{b}_{j}  \big), \quad j \in \{ f, i, o \},
\end{align}
where $\sigma_{j}(\cdot)$, $(\mathbf{W}_{j}, \mathbf{U}_{j})$, and $\mathbf{b}_{j}$ are the activation function, the weight matrices, and the bias vector, respectively.
The forget gate determines what redundant information is discarded; the input gate determines what new information is stored in the internal state; and the output gate determines what information to output.
Once the above three gates are computed, the internal state $\mathbf{c} (n)$ of the LSTM is updated as
\begin{align}
\mathbf{c} (n) & = \mathbf{g}_{f} (n) \odot \mathbf{c} (n-1) \nonumber\\
& \quad + \mathbf{g}_{i} (n) \odot \sigma_{c} \big(  \mathbf{W}_{c} \mathbf{i} (n) + \mathbf{U}_{c} \mathbf{s} (n-1) + \mathbf{b}_{c}  \big)
\end{align}
which determines how much previous state information is kept and how much current state information is allowed.
Then the output of the LSTM is given by
\begin{align}
\mathbf{s} (n) = \mathbf{g}_{o} (n) \odot \sigma_{s} \big(  \mathbf{c} (n)  \big).
\end{align}
